Evaluation of CNN-based Single-Image Depth Estimation Methods

While an increasing interest in deep models for single-image depth estimation methods can be observed, established schemes for their evaluation are still limited. We propose a set of novel quality criteria, allowing for a more detailed analysis by focusing on specific characteristics of depth maps. In particular, we address the preservation of edges and planar regions, depth consistency, and absolute distance accuracy. In order to employ these metrics to evaluate and compare state-of-the-art single-image depth estimation approaches, we provide a new high-quality RGB-D dataset. We used a DSLR camera together with a laser scanner to acquire high-resolution images and highly accurate depth maps. Experimental results show the validity of our proposed evaluation protocol.

==> figures/augmentation/augmented_blur_gaussian.tex <==
\begin{tikzpicture}

  \pgfplotstableread[col sep = comma]{tikz/results_augmented_side/augmented_results_blur.csv}\datatable

  \footnotesize

  \begin{axis}[
ymin = 0,
ymax = 1,
enlargelimits=false,
xmode=log,
%     % legend pos = north east,
%     xmin = 0,
%     xmax = 20,
    ymajorgrids,
    major grid style={lightgray},
%     % axis line style={tumblack},
%     xtick style={draw=none},
    ytick style={draw=none},
%     legend style={draw=tumgray, text=tumblack},
%     legend cell align=left,
%     % legend columns=3,
% %     legend style={at={(0.825,0.95)},anchor=north,/tikz/every even column/.append style={column sep=10}},
% 	legend pos=north east,
    xlabel= $\sigma$,
    ylabel= Error (REL),
    width=.32\linewidth,
    height=.32\linewidth,
%     every axis label/.append style ={tumblack},
%     ytick = {0, 0.05, 0.1},
%     yticklabels={0, 0.05, 0.1},
%     xtick = {0, 5, ..., 20},
%     xmajorgrids,
%     % axis line style={tumgray},
%     % every tick label/.append style={tumgray},
    ylabel near ticks,
%     xlabel near ticks
% yticklabels={},
% xticklabels={},
    ]

    \addplot [mark=none, tumblue, thick] table[x=value, y=eigendnlvgg]{\datatable};
    \addplot [mark=none, tumbluelight, thick] table[x=value, y=eigendnlalex]{\datatable};
    \addplot [mark=none, tumgreen, thick] table[x=value, y=eigen]{\datatable};
    \addplot [mark=none, tumorange, thick] table[x=value, y=fcrn]{\datatable};

  \end{axis}
\end{tikzpicture}


==> figures/augmentation/augmented_noise_gaussian.tex <==
\begin{tikzpicture}

  \pgfplotstableread[col sep = comma]{tikz/results_augmented_side/augmented_results_noise_gaussian.csv}\datatable

  \footnotesize

  \begin{axis}[
ymin = 0,
ymax = 1,
enlargelimits=false,
xmode=log,
%     % legend pos = north east,
%     xmin = 0,
%     xmax = 20,
    ymajorgrids,
    major grid style={lightgray},
%     % axis line style={tumblack},
%     xtick style={draw=none},
    ytick style={draw=none},
%     legend style={draw=tumgray, text=tumblack},
%     legend cell align=left,
%     % legend columns=3,
% %     legend style={at={(0.825,0.95)},anchor=north,/tikz/every even column/.append style={column sep=10}},
% 	legend pos=north east,
    xlabel= $\sigma^2$,
    ylabel= Error (REL),
    width=.32\linewidth,
    height=.32\linewidth,
%     every axis label/.append style ={tumblack},
%     ytick = {0, 0.05, 0.1},
%     yticklabels={0, 0.05, 0.1},
%     xtick = {0, 5, ..., 20},
%     xmajorgrids,
%     % axis line style={tumgray},
%     % every tick label/.append style={tumgray},
    ylabel near ticks,
%     xlabel near ticks
% yticklabels={},
% xticklabels={},
    ]

    \addplot [mark=none, tumblue, thick] table[x=value, y=eigendnlvgg]{\datatable};
    \addplot [mark=none, tumbluelight, thick] table[x=value, y=eigendnlalex]{\datatable};
    \addplot [mark=none, tumgreen, thick] table[x=value, y=eigen]{\datatable};
    \addplot [mark=none, tumorange, thick] table[x=value, y=fcrn]{\datatable};

  \end{axis}
\end{tikzpicture}


==> figures/augmentation/augmented_noise_sp.tex <==
\begin{tikzpicture}

  \pgfplotstableread[col sep = comma]{tikz/results_augmented_side/augmented_results_noise_sp.csv}\datatable

  \footnotesize

  \begin{axis}[
ymin = 0,
ymax = 1,
enlargelimits=false,
xmode=log,
%     % legend pos = north east,
%     xmin = 0,
%     xmax = 20,
    ymajorgrids,
    major grid style={lightgray},
%     % axis line style={tumblack},
%     xtick style={draw=none},
    ytick style={draw=none},
%     legend style={draw=tumgray, text=tumblack},
%     legend cell align=left,
%     % legend columns=3,
% %     legend style={at={(0.825,0.95)},anchor=north,/tikz/every even column/.append style={column sep=10}},
% 	legend pos=north east,
    xlabel= Portion of Affected Pixels,
    ylabel= Error (REL),
    width=.32\linewidth,
    height=.32\linewidth,
%     every axis label/.append style ={tumblack},
%     ytick = {0, 0.05, 0.1},
%     yticklabels={0, 0.05, 0.1},
%     xtick = {0, 5, ..., 20},
%     xmajorgrids,
%     % axis line style={tumgray},
%     % every tick label/.append style={tumgray},
    ylabel near ticks,
%     xlabel near ticks
% yticklabels={},
% xticklabels={},
    ]

    \addplot [mark=none, tumblue, thick] table[x=value, y=eigendnlvgg]{\datatable};
    \addplot [mark=none, tumbluelight, thick] table[x=value, y=eigendnlalex]{\datatable};
    \addplot [mark=none, tumgreen, thick] table[x=value, y=eigen]{\datatable};
    \addplot [mark=none, tumorange, thick] table[x=value, y=fcrn]{\datatable};

  \end{axis}
\end{tikzpicture}


==> figures/augmentation/augmented_results.tex <==
\begin{tikzpicture}

\centering


  \pgfplotstableread[col sep = comma]{tikz/results_augmented_side/augmented_results_blur.csv}\datatableGB
  \pgfplotstableread[col sep = comma]{tikz/results_augmented_side/augmented_results_noise_gaussian.csv}\datatableGN
  \pgfplotstableread[col sep = comma]{tikz/results_augmented_side/augmented_results_noise_sp.csv}\datatableSP

  \footnotesize

  \begin{axis}[
ymin = 0.2,
ymax = 0.8,
enlargelimits=false,
xmode=log,
    ymajorgrids,
    major grid style={lightgray},
    ytick style={draw=none},
    xlabel= $\sigma$ (in \si{\px}),
    ylabel= REL,
    % ylabel near ticks,
    width=.37\linewidth,
    height=.2\linewidth,
name=plot1
    ]
    \addplot [mark=none, tumgreen, thick] table[x=value, y=eigen]{\datatableGB};
    \addplot [mark=none, tumbluelight, thick] table[x=value, y=eigendnlalex]{\datatableGB};
    \addplot [mark=none, tumblue, thick] table[x=value, y=eigendnlvgg]{\datatableGB};
    \addplot [mark=none, tumorange, thick] table[x=value, y=fcrn]{\datatableGB};
  \end{axis}

  \begin{axis}[
  ymin = 0.2,
  ymax = 0.8,
enlargelimits=false,
xmode=log,
    ymajorgrids,
    major grid style={lightgray},
    ytick style={draw=none},
    xlabel= $\sigma^2$ (in \si{\px}),
    % ylabel= Error (REL),
    width=.37\linewidth,
    height=.2\linewidth,
yticklabels={},
legend style={at={(0.48,-0.15)}, anchor=south},
legend style={draw=tumgray, text=tumblack},
% legend cell align=left,
legend columns=4,
name=plot2,
at=(plot1.right of east), anchor= left of west,
    ]
    \addplot [mark=none, tumgreen, thick] table[x=value, y=eigen]{\datatableGN};
    \addplot [mark=none, tumbluelight, thick] table[x=value, y=eigendnlalex]{\datatableGN};
    \addplot [mark=none, tumblue, thick] table[x=value, y=eigendnlvgg]{\datatableGN};
    \addplot [mark=none, tumorange, thick] table[x=value, y=fcrn]{\datatableGN};
  \end{axis}

  \begin{axis}[
  ymin = 0.2,
  ymax = 0.8,
enlargelimits=false,
xmode=log,
    ymajorgrids,
    major grid style={lightgray},
    ytick style={draw=none},
    xlabel= Portion of Affected Pixels,
    % ylabel= Error (REL),
    width=.37\linewidth,
    height=.2\linewidth,
yticklabels={},
name=plot3,
at=(plot2.right of east), anchor=left of west
    ]
    \addplot [mark=none, tumgreen, thick] table[x=value, y=eigen]{\datatableSP};
    \addplot [mark=none, tumbluelight, thick] table[x=value, y=eigendnlalex]{\datatableSP};
    \addplot [mark=none, tumblue, thick] table[x=value, y=eigendnlvgg]{\datatableSP};
    \addplot [mark=none, tumorange, thick] table[x=value, y=fcrn]{\datatableSP};
  \end{axis}

\end{tikzpicture}


==> tikz/results_augmented_side/augmented_table.tex <==
\begin{table*}
 \caption{FIXME: DUMMY TEXT! Results for the augmented dataset. Metric: rel}
 \noteLL[inline]{fix column width or replace by X}
 \label{tab:augmented_results}
 \centering
 \footnotesize
 \begin{tabularx}{\linewidth}{@{}X*{12}{S[table-format=1.3]}@{}}
 \toprule
 \addlinespace

 % Method & \multicolumn{1}{l}{Reference} & \multicolumn{2}{l}{Geometrical} & \multicolumn{3}{l}{Contrast} & \multicolumn{2}{l}{Swapped Channels} & \multicolumn{2}{l}{Hue} & \multicolumn{2}{l}{Saturation} \\
 \scriptsize Method & \multicolumn{1}{l}{\scriptsize Reference} & \multicolumn{2}{l}{\scriptsize Geometrical} & \multicolumn{3}{l}{\scriptsize Contrast} & \multicolumn{2}{l}{\scriptsize Swap Channels} & \multicolumn{2}{l}{\scriptsize Hue (H)} & \multicolumn{2}{l}{\scriptsize Saturation (S)} \\

\cmidrule(lr){3-4} \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(l){12-13}

& & \scriptsize Flip LR & \scriptsize Flip UD & \scriptsize $\gamma = 0.2$ & \scriptsize $\gamma = 2$ & \scriptsize Normalize & \scriptsize GBR & \scriptsize BRG & \scriptsize $+\SI{9}{\degree}$ & \scriptsize $+\SI{90}{\degree}$ & \scriptsize $\times 0.9$ & \scriptsize $\times 0$ \\

\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} \cmidrule(l){12-12} \cmidrule(l){13-13}

\addlinespace

% Eigen DNL (VGG) & 0.000 & 0.271 & 0.425 & 0.398 & 0.302 & 0.288 & 0.293 & 0.299 & 0.288 & 0.294 & 0.287 & 0.288 \\
% FCRN & 0.000 & 0.256 & 0.436 & 0.353 & 0.301 & 0.273 & 0.279 & 0.282 & 0.274 & 0.278 & 0.273 & 0.274 \\
% Eigen DNL (AlexNet) & 0.000 & 0.306 & 0.431 & 0.429 & 0.349 & 0.359 & 0.340 & 0.326 & 0.319 & 0.340 & 0.317 & 0.318 \\
% Eigen & 0.000 & 0.336 & 0.428 & 0.419 & 0.379 & 0.359 & 0.380 & 0.370 & 0.361 & 0.385 & 0.359 & 0.360 \\

\scriptsize Eigen                  &    0.360    &    -0.024    &    0.068    &    0.059    &    0.019    &    -0.001    &    0.020    &    0.010    &    0.010    &    0.025     &    -0.001   &    0.000 \\
\scriptsize Eigen DNL (AlexNet)    &    0.318    &    -0.012    &    0.113    &    0.111    &    0.031    &    0.041    &    0.022    &    0.008    &    0.005    &    0.022     &    -0.001   &    0.000 \\
\scriptsize Eigen DNL (VGG)        &    0.288    &    -0.017    &    0.137    &    0.110    &    0.014    &    0.000    &    0.005    &    0.011    &    0.002    &    0.006     &    -0.001   &    0.000 \\
\scriptsize FCRN                   &    0.274    &    -0.018    &    0.162    &    0.079    &    0.027    &    -0.001    &    0.005    &    0.008                  &    0.001     &    0.004    &    -0.001   &    0.000 \\



%
%
%  Method & \multicolumn{2}{l}{Geometrical} & \multicolumn{3}{l}{Contrast} & \multicolumn{7}{l}{Gaussian Blur ($\sigma = 10^{x}$)} \\
%  \cmidrule(r){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(l){7-13}
%  & \multicolumn{1}{l}{\footnotesize Flip LR} & \footnotesize Flip UD & \footnotesize $\gamma = 0.2$ & \footnotesize $\gamma = 2$ & \footnotesize Stretched & \footnotesize -0.5 & \footnotesize -0.25 & \footnotesize 0 & \footnotesize 0.25 & \footnotesize 0.5 & \footnotesize 0.75 & \footnotesize 1 \\
%  \addlinespace
% FCRN & 0.256 & 0.436 & 0.353 & 0.301 & 0.273 & 0.274 & 0.279 & 0.29 & 0.313 & 0.641 & 0.407 & 0.602 \\
% Eigen DNL (AlexNet) & 0.306 & 0.431 & 0.429 & 0.349 & 0.359 & 0.318 & 0.322 & 0.338 & 0.401 & 0.715 & 0.495 & 0.635 \\
% Eigen & 0.336 & 0.428 & 0.419 & 0.379 & 0.359 & 0.36 & 0.364 & 0.381 & 0.435 & 0.587 & 0.498 & 0.551 \\
%  % Method & \multicolumn{2}{l}{Geometrical} & \multicolumn{3}{l}{Contrast ($\gamma$)} & \multicolumn{7}{l}{Gaussian Blur ($\sigma = 10^{x}$)} & \multicolumn{7}{l}{Swapped Channels} & \multicolumn{9}{l}{Hue} & \multicolumn{9}{l}{Saturation} & \multicolumn{9}{l}{Gaussian Noise} & \multicolumn{9}{l}{Salt \& Pepper Noise} \\
%  % & Flip LR & Flip UD & 0.2 & 2 & Stretched & -0.5 & -0.25 & 0 & 0.25 & 0.5 & 0.75 & 1 & GBR & BRG & $\frac{10^{-1} \cdot 9}{360}$ & $\frac{10^{-0.75} \cdot 9}{360}$ & $\frac{10^{-0.5} \cdot 9}{360}$ & $\frac{10^{-0.25} \cdot 9}{360}$ & $\frac{10^{0} \cdot 9}{360}$ & $\frac{10^{0.25} \cdot 9}{360}$ & $\frac{10^{0.5} \cdot 9}{360}$ & $\frac{10^{0.75} \cdot 9}{360}$ & $\frac{10^{1} \cdot 9}{360}$ & $1 - 10^{-2}$ & $1 - 10^{-1.75}$ & $1 - 10^{-1.5}$ & $1 - 10^{-1.25}$ & $1 - 10^{-1}$ & $1 - 10^{-0.75}$ & $1 - 10^{-0.5}$ & $1 - 10^{-0.25}$ & $1 - 10^{0}$ & $\sigma^2 = 10^{-4}$ & $\sigma^2 = 10^{-3.5}$ & $\sigma^2 = 10^{-3}$ & $\sigma^2 = 10^{-2.5}$ & $\sigma^2 = 10^{-2}$ & $\sigma^2 = 10^{-1.5}$ & $\sigma^2 = 10^{-1}$ & $\sigma^2 = 10^{-0.5}$ & $\sigma^2 = 10^{0}$ & $10^{-4} \cdot 0.5$ & $10^{-3.5} \cdot 0.5$ & $10^{-3} \cdot 0.5$ & $10^{-2.5} \cdot 0.5$ & $10^{-2} \cdot 0.5$ & $10^{-1.5} \cdot 0.5$ & $10^{-1} \cdot 0.5$ & $10^{-0.5} \cdot 0.5$ & $10^{0} \cdot 0.5$ \\
%
%  Eigen DNL (VGG) & 0.271 & 0.425 & 0.398 & 0.302 & 0.288 & 0.288 & 0.295 & 0.31 & 0.342 & 0.679 & 0.389 & 0.51 \\
%  % Method & \multicolumn{9}{l}{Gaussian Blur} & \multicolumn{2}{l}{Color Channels} & \multicolumn{9}{l}{Hue} & \multicolumn{9}{l}{Saturation} & \multicolumn{2}{l}{Gamma} & Contrast & \multicolumn{2}{l}{Flip} & \multicolumn{11}{l}{Gaussian Noise} & \multicolumn{11}{l}{Salt \& Pepper Noise} \\
%  % % Method & blur gaussian 0 & blur gaussian 1 & blur gaussian 2 & blur gaussian 3 & blur gaussian 4 & blur gaussian 5 & blur gaussian 6 & blur gaussian 7 & blur gaussian 8 & color flip 0 & color flip 1 & color hue 0 & color hue 1 & color hue 2 & color hue 3 & color hue 4 & color hue 5 & color hue 6 & color hue 7 & color hue 8 & color sat 0 & color sat 1 & color sat 2 & color sat 3 & color sat 4 & color sat 5 & color sat 6 & color sat 7 & color sat 8 & contrast gamma 0 & contrast gamma 1 & contrast stretch 0 & flip lr 0 & flip ud 0 & noise gaussian 0 & noise gaussian 1 & noise gaussian 2 & noise gaussian 3 & noise gaussian 4 & noise gaussian 5 & noise gaussian 6 & noise gaussian 7 & noise gaussian 8 & noise gaussian 9 & noise gaussian 10 & noise sp 0 & noise sp 1 & noise sp 2 & noise sp 3 & noise sp 4 & noise sp 5 & noise sp 6 & noise sp 7 & noise sp 8 & noise sp 9 & noise sp 10 \\
%  % \addlinespace
%  % eigendnlvgg & 2.59 & 2.59 & 2.6 & 2.64 & 2.74 & 2.91 & 4.26 & 3.12 & 3.6 & 2.59 & 2.63 & 2.6 & 2.6 & 2.6 & 2.6 & 2.61 & 2.6 & 2.62 & 2.6 & 2.61 & 2.58 & 2.58 & 2.58 & 2.59 & 2.59 & 2.59 & 2.59 & 2.59 & 2.59 & 3.11 & 2.65 & 2.59 & 2.47 & 3.23 & 2.59 & 2.6 & 2.6 & 2.61 & 2.63 & 2.69 & 2.84 & 3.16 & 3.71 & 4.1 & 4.17 & 2.59 & 2.59 & 2.59 & 2.6 & 2.6 & 2.61 & 2.64 & 2.73 & 2.94 & 3.49 & 4.16 \\
%  % fcrn & 2.42 & 2.42 & 2.42 & 2.44 & 2.5 & 2.64 & 4.07 & 3.14 & 3.94 & 2.46 & 2.46 & 2.42 & 2.42 & 2.42 & 2.42 & 2.42 & 2.42 & 2.43 & 2.42 & 2.46 & 2.46 & 2.42 & 2.41 & 2.41 & 2.41 & 2.41 & 2.41 & 2.41 & 2.42 & 2.92 & 2.53 & 2.41 & 2.27 & 3.22 & 2.42 & 2.42 & 2.42 & 2.43 & 2.44 & 2.49 & 2.64 & 3.07 & 3.61 & 3.87 & 3.85 & 2.42 & 2.42 & 2.41 & 2.42 & 2.42 & 2.43 & 2.45 & 2.53 & 2.76 & 3.42 & 3.86 \\
%  % eigendnlalex & 2.63 & 2.63 & 2.63 & 2.67 & 2.79 & 3.09 & 4.36 & 3.5 & 4.05 & 2.66 & 2.63 & 2.63 & 2.63 & 2.64 & 2.63 & 2.65 & 2.63 & 2.66 & 2.64 & 2.68 & 2.62 & 2.62 & 2.61 & 2.62 & 2.62 & 2.63 & 2.63 & 2.63 & 2.63 & 3.27 & 2.76 & 2.9 & 2.51 & 3.15 & 2.63 & 2.63 & 2.63 & 2.63 & 2.64 & 2.66 & 2.75 & 2.92 & 3.16 & 3.48 & 3.7 & 2.63 & 2.63 & 2.63 & 2.63 & 2.63 & 2.63 & 2.64 & 2.67 & 2.8 & 3.05 & 3.51 \\
%  % eigen & 2.91 & 2.91 & 2.91 & 2.95 & 3.06 & 3.34 & 3.98 & 3.62 & 3.85 & 2.99 & 2.95 & 2.91 & 2.91 & 2.94 & 2.91 & 2.97 & 2.91 & 3.02 & 2.92 & 3.04 & 2.92 & 2.9 & 2.9 & 2.9 & 2.9 & 2.91 & 2.91 & 2.91 & 2.91 & 3.3 & 3.01 & 2.9 & 2.74 & 3.23 & 2.91 & 2.91 & 2.91 & 2.91 & 2.92 & 2.94 & 2.99 & 3.11 & 3.34 & 3.63 & 3.85 & 2.91 & 2.91 & 2.91 & 2.91 & 2.91 & 2.91 & 2.92 & 2.94 & 3.01 & 3.23 & 3.68 \\
 \addlinespace
 \bottomrule
 \end{tabularx}
\end{table*}


==> tikz/results_augmented_side/augmented_table_created.tex <==
\begin{table*} 
 \caption{FIXME: DUMMY TEXT! Results for the augmented dataset. Metric: thr125} 
 \label{tab:augmented_results} 
 \centering 
 \tiny 
 \begin{tabularx}{\linewidth}{@{}lXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX@{}} 
 \toprule 
 \addlinespace 
 Method & blur gaussian 0 & blur gaussian 1 & blur gaussian 2 & blur gaussian 3 & blur gaussian 4 & blur gaussian 5 & blur gaussian 6 & blur gaussian 7 & blur gaussian 8 & color flip 0 & color flip 1 & color hue 0 & color hue 1 & color hue 2 & color hue 3 & color hue 4 & color hue 5 & color hue 6 & color hue 7 & color hue 8 & color sat 0 & color sat 1 & color sat 2 & color sat 3 & color sat 4 & color sat 5 & color sat 6 & color sat 7 & color sat 8 & contrast gamma 0 & contrast gamma 1 & contrast stretch 0 & flip lr 0 & flip ud 0 & noise gaussian 0 & noise gaussian 1 & noise gaussian 2 & noise gaussian 3 & noise gaussian 4 & noise gaussian 5 & noise gaussian 6 & noise gaussian 7 & noise gaussian 8 & noise gaussian 9 & noise gaussian 10 & noise sp 0 & noise sp 1 & noise sp 2 & noise sp 3 & noise sp 4 & noise sp 5 & noise sp 6 & noise sp 7 & noise sp 8 & noise sp 9 & noise sp 10 \\ 
 \addlinespace 
 eigendnlvgg & 0.469 & 0.469 & 0.468 & 0.446 & 0.401 & 0.308 & 0.039 & 0.22 & 0.108 & 0.464 & 0.438 & 0.469 & 0.469 & 0.464 & 0.468 & 0.457 & 0.469 & 0.449 & 0.467 & 0.458 & 0.475 & 0.478 & 0.477 & 0.475 & 0.474 & 0.471 & 0.47 & 0.469 & 0.469 & 0.177 & 0.437 & 0.465 & 0.431 & 0.204 & 0.469 & 0.467 & 0.465 & 0.456 & 0.433 & 0.381 & 0.284 & 0.172 & 0.099 & 0.055 & 0.049 & 0.469 & 0.47 & 0.47 & 0.469 & 0.467 & 0.461 & 0.44 & 0.352 & 0.241 & 0.116 & 0.048 \\ 
 fcrn & 0.555 & 0.555 & 0.554 & 0.545 & 0.523 & 0.443 & 0.052 & 0.254 & 0.066 & 0.536 & 0.53 & 0.555 & 0.555 & 0.55 & 0.554 & 0.544 & 0.555 & 0.541 & 0.553 & 0.531 & 0.532 & 0.551 & 0.557 & 0.558 & 0.558 & 0.556 & 0.556 & 0.555 & 0.555 & 0.34 & 0.486 & 0.555 & 0.528 & 0.197 & 0.554 & 0.553 & 0.553 & 0.546 & 0.53 & 0.49 & 0.407 & 0.276 & 0.134 & 0.08 & 0.085 & 0.555 & 0.556 & 0.556 & 0.559 & 0.551 & 0.544 & 0.528 & 0.475 & 0.355 & 0.167 & 0.083 \\ 
 eigendnlalex & 0.424 & 0.424 & 0.424 & 0.397 & 0.328 & 0.188 & 0.029 & 0.107 & 0.05 & 0.389 & 0.402 & 0.424 & 0.423 & 0.421 & 0.423 & 0.416 & 0.422 & 0.41 & 0.422 & 0.391 & 0.438 & 0.439 & 0.439 & 0.436 & 0.433 & 0.43 & 0.427 & 0.426 & 0.426 & 0.169 & 0.358 & 0.352 & 0.398 & 0.249 & 0.424 & 0.425 & 0.425 & 0.426 & 0.426 & 0.42 & 0.38 & 0.342 & 0.274 & 0.177 & 0.126 & 0.425 & 0.425 & 0.425 & 0.425 & 0.427 & 0.429 & 0.432 & 0.426 & 0.398 & 0.339 & 0.169 \\ 
 eigen & 0.349 & 0.349 & 0.349 & 0.332 & 0.275 & 0.165 & 0.075 & 0.114 & 0.087 & 0.326 & 0.336 & 0.349 & 0.348 & 0.338 & 0.348 & 0.326 & 0.346 & 0.306 & 0.344 & 0.3 & 0.369 & 0.367 & 0.365 & 0.358 & 0.354 & 0.352 & 0.351 & 0.35 & 0.35 & 0.214 & 0.313 & 0.352 & 0.34 & 0.241 & 0.349 & 0.349 & 0.348 & 0.347 & 0.345 & 0.338 & 0.324 & 0.284 & 0.212 & 0.131 & 0.084 & 0.349 & 0.349 & 0.349 & 0.349 & 0.349 & 0.348 & 0.345 & 0.342 & 0.317 & 0.247 & 0.12 \\ 
 \addlinespace 
 \bottomrule 
 \end{tabularx} 
\end{table*}
